Computational homogenization of higher-order continua

We introduce a novel computational framework for the multiscale simulation of higher-order continua that allows for the consideration of first-, second- and third- order effects at both micro- and macro-level. In line with classical two-scale approaches, we describe the microstructure via representative volume elements (RVE) that are attached at each integration point of the macroscopic problem. To take account of the extended continuity requirements of independent fields at micro- and macro-level, we discretize both scales via isogeometric analysis (IGA). As a result, we obtain an IGA2-method that is conceptually similar to the well-known FE2-method. We demonstrate the functionality and accuracy of this novel multiscale method by means of a series of multiscale simulations involving different kinds of higher-order continua.

==> preamble.tex <==
% !TeX root = MAIN.tex


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Packages
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage[english]{babel}
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\usepackage{amsfonts,amsmath,amsthm,amssymb}
\usepackage{mathtools}
\usepackage{hyperref}
\usepackage{autonum}
%\usepackage[normalem]{ulem}
%\usepackage{ulem}
\usepackage{hhline}
\usepackage{array}
%\usepackage{gensymb}
\usepackage{diagbox}
\usepackage{tcolorbox}
\usepackage{mdframed}
\usepackage{multicol}
\usepackage{subcaption}
%\usepackage[labelfont=bf,font=sf]{caption}
\usepackage{moreverb}
\usepackage{bbm}
\usepackage{placeins}
\usepackage{enumerate}


%\usepackage{todonotes}
\allowdisplaybreaks
%\usepackage[breaklinks=true]{hyperref}
%\usepackage{breakcites}


% --- biblio ----

%\usepackage[doi=false,isbn=false,url=false]{natbib}
%\usepackage{natbib}
%%	\bibliographystyle{ieeetr}
%\bibliographystyle{abbrvnat}	
%\setcitestyle{authoryear, square}
%\renewcommand{\cite}[1]{((\citet{#1}))}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TIKZ
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{tikz}
\usetikzlibrary{decorations.pathmorphing} % for snake lines
\usetikzlibrary{matrix} % for block alignment
\usetikzlibrary{arrows} % for arrow heads
\usetikzlibrary{calc} % for manimulation of coordinates
\usetikzlibrary{shapes}
\usetikzlibrary{shapes.geometric}

% TikZ styles for drawing
\tikzstyle{block} = [draw,rectangle,thick,minimum height=2em,minimum width=2em]
\tikzstyle{sum} = [draw,circle,inner sep=0mm,minimum size=2mm]
\tikzstyle{connector} = [->,thick]
\tikzstyle{line} = [thick]
\tikzstyle{branch} = [circle,inner sep=0pt,minimum size=1mm,fill=black,draw=black]
\tikzstyle{guide} = []
\tikzstyle{snakeline} = [connector, decorate, decoration={pre length=0.2cm,
	post length=0.2cm, snake, amplitude=.4mm,
	segment length=2mm},thick, magenta, ->]

\usepackage{pgfplots}
%%\usepackage{pgffor}
%\usepackage{pgfplotstable}
%\usepgfplotslibrary{colorbrewer}
%\usepgfplotslibrary{groupplots}
%%\pgfplotsset{compat=1.15}
%\pgfplotsset{compat=newest}
%\usepackage{tikz}
%\usetikzlibrary{external}
%\tikzexternalize[prefix=tikz/]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Notations 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% math
\newcommand{\X}{\vec{X}}
\newcommand{\x}{\vec{x}}
\newcommand{\y}{\vec{y}}
\newcommand{\z}{\vec{z}}
\newcommand{\Id}{\operatorname*{Id}}
\newcommand{\sign}{\operatorname*{sign}}
\newcommand{\op}[1]{\operatorname*{#1}}
\newcommand{\eps}{\varepsilon}
\newcommand{\J}{\mathcal{J}}
\newcommand{\dev}[1]{\text{dev}\left[#1\right]}
\newcommand{\norm}[1]{\lVert #1 \rVert}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\dt}{\Delta t}
\newcommand{\dx}{\Delta x}
\newcommand{\sgn}[1]{\ \text{sgn}\left(#1\right) }
\newcommand{\sca}[2]{\langle #1, \; #2 \rangle}
\newcommand{\frc}[2]{{\textstyle\frac{#1}{#2}}}
\newcommand{\minus}{\scalebox{0.7}[1.0]{\( - \)}}
\newcommand{\inv}{^{\scalebox{0.7}[1.0]{\( - \)}1}}%{^{-1}}
\newcommand{\tp}{^\intercal}
\newcommand{\tpc}{^*}
\renewcommand{\exp}[1]{e^{#1}}
\newcommand{\Exp}[1]{\operatorname*{Exp}\left(#1\right)}
\renewcommand{\i}{\mathrm{i}}
\renewcommand{\d}{\operatorname{d}\!}
\newcommand{\tr}{\operatorname{tr}}
\renewcommand{\Re}{\mathfrak{Re}}
\renewcommand{\Im}{\mathfrak{Im}}
\newcommand{\B}{\lbrace -1, 1\rbrace}
\newcommand{\Ind}{\mathbbm{1}}
\renewcommand{\O}{\mathcal{O}}

% vectors and matrices
\newcommand{\mat}[1]{\begin{bmatrix} #1 \end{bmatrix}}
\newcommand{\diag}{\operatorname{diag}}
\renewcommand{\vec}[1]{\pmb{#1}}
\newcommand{\vct}[1]{\vec{#1}}
\newcommand{\ten}[1]{\pmb{#1}}
\newcommand{\tns}[1]{\ten{#1}}
\newcommand{\tnsfour}[1]{\pmb{#1}}

% parantheses
\newcommand{\bbc}[1]{\left( #1 \right)}
\newcommand{\rbc}[1]{\left[ #1 \right]}

% differentiation
\newcommand{\drv}[2]{\frac{\partial #1}{\partial #2}} %{\partial_{#1} #2}
\newcommand{\D}[2]{\partial_{#1} #2}
\renewcommand{\div}{\nabla\cdot}
\newcommand{\grad}{\nabla}
\newcommand{\gradS}{\nabla\!_s}
\newcommand{\Jac}[2][]{ \operatorname*{D_{#1}}\! #2  }
\newcommand{\Hess}[1]{ D^2#1  }


% integral transforms
\newcommand{\La}[1]{\mathfrak{L}\lbrace #1 \rbrace }
\newcommand{\Lai}[1]{\mathfrak{L}\inv\lbrace #1 \rbrace }
\newcommand{\F}{\mathcal{F}} % Fourrier transform
\newcommand{\Fi}{\mathcal{F}^{-1}} % inverse Fourrier transform
\newcommand{\FFT}[1]{\operatorname{FFT}\left\lbrace #1 \right\rbrace} % Discrete (Fast) Fourrier Transform
\newcommand{\IFFT}[1]{\operatorname{IFFT}\left\lbrace #1 \right\rbrace} % inverse Discrete (Fast) Fourrier Transform

% Sets
\newcommand{\Z}{\mathbb{Z}} % integer
\newcommand{\R}{\mathbb{R}} % real
\newcommand{\C}{\mathbb{C}} % complex
\newcommand{\N}{\mathbb{N}} % natural

% Matrix groups
\newcommand{\SymM}[1][3]{\op{S}^{#1}} % Symmetric matrices
\newcommand{\PSD}[1][3]{\SymM[#1]_+} % Symmetric positive semi-definite matrices
\newcommand{\PD}[1][3]{\SymM[#1]_{++}}  % Symmetric positive definite matrices
\newcommand{\SO}[1]{\operatorname{SO}_{#1}}  % Symmetric positive definite matrices

% Spaces
\newcommand{\HS}{\mathcal{H}} % Hilbert space
\newcommand{\K}{\mathcal{K}} % Krylov subspace
\renewcommand{\L}[1]{\op{L}^{\!#1}} % Lesbegues space
\newcommand{\W}[2]{\op{W}^{#1,#2}} % Sobolev space
\renewcommand{\H}[1]{\op{H}^{#1}} % Sobolev space
\newcommand{\Cn}[1]{\op{C}^{#1}} % Sobolev space
%\newcommand{\M}{\mathbb{M}} % Space of matrices
\newcommand{\vspan}{\op{span}} % convex hull (span)

% Probability
\newcommand{\E}[1]{\operatorname{\mathbb{E}}\rbc{#1}}
\newcommand{\Prob}[1]{\operatorname{\mathbb{P}}\rbc{#1}}
\newcommand{\Var}[1]{\operatorname{Var}\rbc{#1}}
\newcommand{\Gaussian}{\mathcal{N}}
\newcommand{\Cov}{\tns{C}}
\newcommand{\WN}{\mathcal{W}} % White noise
\newcommand{\WNhat}{\hat{\mathcal{W}}} % Fourier of White noise


% Special functions
\newcommand{\BesselJ}[1]{\mathcal{J}_{#1}}
\newcommand{\BesselK}[1]{\mathcal{K}_{#1}}
\newcommand{\erf}{\operatorname{erf}}
\newcommand{\erfc}{\operatorname{erfc}}
\newcommand{\hypTwoOne}{{\;}_{2}F_{1}}


% raccourcis
\newcommand{\MatLab}{MatLab R2016b}

% formating
\newcounter{rownumber}
\newcommand{\rownumber}{\stepcounter{rownumber}\therownumber}


% Elasticity problem
\newcommand{\dir}{\vec{e}}
\newcommand{\disp}{\vec{u}}
\newcommand{\strain}{\tns{\varepsilon}}
\newcommand{\stress}{\tns{\sigma}}
\newcommand{\Macrostrain}{\tns{E}}%{\bar{\strain}}
\newcommand{\Macrostress}{\tns{\Sigma}}%{\bar{\stress}}
\newcommand{\dv}{\tns{s}}
\newcommand{\nbhd}{O}
\newcommand{\thickness}{t}
\newcommand{\bulk}{K}
\newcommand{\shear}{G}
\newcommand{\Stiffness}{\tnsfour{C}}
\newcommand{\QoI}{Q}


% Fiber coupling
\newcommand{\stiffnessC}{\ten{C}}%{\ten{\mathfrak{C}}}
\newcommand{\stiffnessD}{\ten{D}}%{\ten{\mathfrak{D}}}
\newcommand{\ds}[1]{\drv{#1}{s}} % derivative along fiber
\newcommand{\axl}{\operatorname{axl}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%    Theorem envs
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{rmk}{Remark}
\newtheorem{lemma}{Lemma}
%\newdefinition{}{Remark}
%\newtheorem{corollary}{Corollary}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%    Revision
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\myRed}{\color{red!70!black}}
\newcommand{\rev}[1]{{\color{red} #1}}








==> sections/IGAsquare.tex <==

\section{Introduction}

Whether or not morphological features of a material are visible depends on the observed length scale. While a material may appear perfectly homogeneous at one scale, it may be heterogeneous at another. A typical example for such a scenario is a composite, whose phases are distinguishable only at a small length scale and whose heterogeneous properties are linked to homogeneous properties at a larger scale. In general, the involved length scales are considered \textit{separated} if the contrast between the microscopic and the macroscopic length scale is sufficiently high.%
\footnote{%
More strictly speaking, separation of scales is present when the wavelengths of physical fields at the higher scale are very much larger than the dimensions of heterogeneities at the lower scale
(\cite{sanchez-palencia_homogenization_1983}).
}
In such cases, it is reasonable to describe the homogenized, macroscopic behavior with classical, first-order theories. In contrast to that, when the scales are not clearly separated, the description of the macroscopic behavior needs to be based on generalized, higher-order theories.

Generalized theories for materials are nowadays well-established. They trace back to the seminal work of
\cite{cosserat_theorie_1909},
who investigated the emergence and significance of couple stresses for the modeling of the size-dependent response of materials more than a hundred years ago. In their theory, the Cosserat brothers linked \textit{couple stresses} to the gradient of a microscopic rotation field and classical \textit{force stresses} to the gradient of the macroscopic translation field (i.e., the displacements). In that context, the microscopic rotation field is understood independent from the macroscopic rotation field. An extended theory based on the consideration of both macroscopic translational and macroscopic rotational degrees of freedom was later developed by
\cite{toupin_elastic_1962,toupin_theories_1964,mindlin_effects_1962}.
We refer to
\cite{altenbach_cosserat_2013}
and
\cite{ehlers_cosserat_2020}
for rigorous expositions of the Cosserats' couple-stress theory as well as to
\cite{eringen_mechanics_1968,eringen_microcontinuum_2012,hadjesfandiari_couple_2011}
for further developments and generalizations.

Next to classical couple-stress theories, there exist a number of further approaches to the modeling of size effects in materials. An important branch is given by so-called \textit{strain-gradient theories}, which for linear elastic solids have first been proposed by
\cite{mindlin_micro-structure_1964}.
Associated theories are based on the incorporation of higher-order gradients of the displacement field into the material description. We refer to
\cite{mindlin_first_1968}
for further specifications based on the first gradient of strain and to
\cite{mindlin_second_1965}
for an extension involving the second gradient of strain. The interested reader is further referred to
\cite{germain_method_1973}
and
\cite{kirchner_unifying_2005}
for underlying virtual-work and variational principles, respectively, to
\cite{javili_geometrically_2013}
for extensions towards fully nonlinear settings, and to
\cite{zervos_finite_2008,askes_gradient_2011,fischer_isogeometric_2011}
for possible numerical implementations. A general overview of gradient-extended continua is available through the monographs of
\cite{maugin_mechanics_2010,altenbach_mechanics_2011,bertram_mechanics_2020}.
Next to gradient-theories for elastic materials, there exists a rich theory on gradient-extended models for dissipative solids. In these cases, the gradient extensions are classicaly linked to internal variables like the plastic strains
(\cite{aifantis_physics_1987,fleck_strain_1994})
and the damage field
(\cite{peerlings_gradient_1996}).
We refer to
\cite{miehe_multi-field_2011}
for an associated variational treatment.

The above mentioned formulations have in common that they incorporate the notion of microstructure (and its size) in a phenomenological way. In contrast to that, microstructural information about morhology and material properties can be accounted for in an explicit manner by means of \textit{homogenization methods}. As in case of phenomenological material modeling, size effects may be incorporated in related schemes, depending on the existence of scale separation. If the considered scales are clearly separated, \textit{classical} or \textit{first-order} homogenization schemes are applicable; if they are not, \textit{generalized} or \textit{higher-order} schemes become necessary.

In the context of first-order homogenization schemes, we refer to
\cite{hill_elastic_1952,hashin_variational_1963,hill_self-consistent_1965,mori_average_1973,willis_bounds_1977}
for fundamental analytical approaches and to
\cite{smit_prediction_1998,miehe_computational_1999-1,feyel_fe2_2000,kouznetsova_approach_2001}
for seminal contributions to two-scale numerical simulations. In the context of higher-order and generalized continua, analytical approaches have been explored by
\cite{diener_bounds_1984,gambin_higher-order_1989,boutin_microstructural_1996,drugan_micromechanics-based_1996},
see also the overview by
\cite{forest_homogenization_2002}
as well as the more recent contributions of
\cite{hutter_homogenization_2017,ganghoffer_variational_2021}.
Associated computational homogenization schemes have been developed in the framework of couple-stress and micromorphic theories by
\cite{bouyge_micromechanically_2001,feyel_multilevel_2003,janicke_two-scale_2009,rokos_micromorphic_2019,ALAVI2021104278}
and in the framework of macroscopic strain-gradient approaches by
\cite{kouznetsova_multi-scale_2002,kouznetsova_multi-scale_2004,bacigalupo_second-order_2010,yvonnet_computational_2020,Maurice2019,Ganghoffer2019}.
We refer to
\cite{forest_cosserat_1998,forest_generalized_2011}
for seminal treatments. 

The present work is devoted to the \textit{multiscale computational homogenization of gradient-extended continua} and unites ingredients of the works of
\cite{kouznetsova_multi-scale_2002}
with respect to the gradient extensions at the homogenized \MK{macroscale}, of
\cite{miehe_computational_1999}
with regard to the algorithmic linearization of the macroscopic field equations, and of
\cite{cirak_subdivision_2000,hughes_isogeometric_2005}
with regard to spatial discretizations. In contast to the contribution of
\cite{kouznetsova_multi-scale_2002},
which combines a Cauchy continuum at the lower length scale \MK{(from now on denoted as microscale, representing the microstructure at each material point)} with a gradient-extended continuum at the larger \MK{macroscale}, we will take into account \textit{gradient-extended continua at both scales}.  \MK{Gradient-extended continua on the microscale can be taken into account, e.g.\ if embedded fibers on this scale are considered as continuum degenerated continua,  see \cite{khristenko2021,Schulte2020b} with analytical, numerical and experimental details on this prototypical example.} This endeavor poses additional challenges not only for the theoretical treatment, but also for the numerical implementation. The latter is due to the fact that the gradient extensions come along with the requirement of $C^1$-continuous approximations of independent fields at both scales. Such a requirement can be captured in an elegant way by employing \textit{isogeometric analysis} in the sense of
\cite{cirak_subdivision_2000,hughes_isogeometric_2005}.
A further algorithmic feature of the proposed implementation is due to the linearization of the macroscopic boundary value problem. Here, we employ the approach advocated by
\cite{miehe_computational_1999},
which was originally developed for first-order homogenization. As we will see, the associated gradient extensions result in settings that remind of the linearized structures appearing in the coupled homogenization schemes considered by
\cite{schroder_two-scale_2012,keip_two-scale_2014,keip_multiscale_2016}.


==> sections/introduction.tex <==
\section{Introduction}

Whether or not morphological features of a material are visible depends on the observed length scale. While a material may appear perfectly homogeneous at one scale, it may be heterogeneous at another. A typical example for such a scenario is a composite, whose phases are distinguishable only at a small length scale and whose heterogeneous properties are linked to homogeneous properties at a larger scale. In general, the involved length scales are considered \textit{separated} if the contrast between the microscopic and the macroscopic length scale is sufficiently high.%
\footnote{%
More strictly speaking, separation of scales is present when the wavelengths of physical fields at the higher scale are very much larger than the dimensions of heterogeneities at the lower scale
(\cite{sanchez-palencia_homogenization_1983}).
}
In such cases, it is reasonable to describe the homogenized, macroscopic behavior with classical, first-order theories. In contrast to that, when the scales are not clearly separated, the description of the macroscopic behavior needs to be based on generalized, higher-order theories.

Generalized theories for materials are nowadays well-established. They trace back to the seminal work of
\cite{cosserat_theorie_1909},
who investigated the emergence and significance of couple stresses for the modeling of the size-dependent response of materials more than a hundred years ago. In their theory, the Cosserat brothers linked \textit{couple stresses} to the gradient of a microscopic rotation field and classical \textit{force stresses} to the gradient of the macroscopic translation field (i.e., the displacements). In that context, the microscopic rotation field is understood independent from the macroscopic rotation field. An extended theory based on the consideration of both macroscopic translational and macroscopic rotational degrees of freedom was later developed by
\cite{toupin_elastic_1962,toupin_theories_1964,mindlin_effects_1962}.
We refer to
\cite{altenbach_cosserat_2013}
and
\cite{ehlers_cosserat_2020}
for rigorous expositions of the Cosserats' couple-stress theory as well as to
\cite{eringen_mechanics_1968,eringen_microcontinuum_2012,hadjesfandiari_couple_2011}
for further developments and generalizations.

Next to classical couple-stress theories, there exist a number of further approaches to the modeling of size effects in materials. An important branch is given by so-called \textit{strain-gradient theories}, which for linear elastic solids have first been proposed by
\cite{mindlin_micro-structure_1964}.
Associated theories are based on the incorporation of higher-order gradients of the displacement field into the material description. We refer to
\cite{mindlin_first_1968}
for further specifications based on the first gradient of strain and to
\cite{mindlin_second_1965}
for an extension involving the second gradient of strain. The interested reader is further referred to
\cite{germain_method_1973}
and
\cite{kirchner_unifying_2005}
for underlying virtual-work and variational principles, respectively, to
\cite{javili_geometrically_2013}
for extensions towards fully nonlinear settings, and to
\cite{zervos_finite_2008,askes_gradient_2011,fischer_isogeometric_2011}
for possible numerical implementations. A general overview of gradient-extended continua is available through the monographs of
\cite{maugin_mechanics_2010,altenbach_mechanics_2011,bertram_mechanics_2020}.  Khristenko et al.\ \cite{khristenko2021} demonstrates, that embedded beams generate an anisotropic second gradient formulation,  representing bending and torsion of the beam within the matrix material. Next to gradient-theories for elastic materials, there exists a rich theory on gradient-extended models for dissipative solids. In these cases, the gradient extensions are classicaly linked to internal variables like the plastic strains
(\cite{aifantis_physics_1987,fleck_strain_1994})
and the damage field
(\cite{peerlings_gradient_1996}).
We refer to
\cite{miehe_multi-field_2011}
for an associated variational treatment.

The above mentioned formulations have in common that they incorporate the notion of microstructure (and its size) in a phenomenological way. In contrast to that, microstructural information about morphology and material properties can be accounted for in an explicit manner by means of \textit{homogenization methods}. As in case of phenomenological material modeling, size effects may be incorporated in related schemes, depending on the existence of scale separation. If the considered scales are clearly separated, \textit{classical} or \textit{first-order} homogenization schemes are applicable; if they are not, \textit{generalized} or \textit{higher-order} schemes become necessary.

In the context of first-order homogenization schemes, we refer to
\cite{hill_elastic_1952,hashin_variational_1963,hill_self-consistent_1965,mori_average_1973,willis_bounds_1977}
for fundamental analytical approaches and to
\cite{smit_prediction_1998,miehe_computational_1999-1,feyel_fe2_2000,kouznetsova_approach_2001}
for seminal contributions to two-scale finite-element (FE) simulations. In the context of higher-order and generalized continua, analytical approaches have been explored by
\cite{diener_bounds_1984,gambin_higher-order_1989,boutin_microstructural_1996,drugan_micromechanics-based_1996},
see also the overview by
\cite{forest_homogenization_2002}
as well as the more recent contributions of
\cite{hutter_homogenization_2017,ganghoffer_variational_2021}.
Associated computational homogenization schemes have been developed in the framework of couple-stress and micromorphic theories by
\cite{bouyge_micromechanically_2001,feyel_multilevel_2003,janicke_two-scale_2009,rokos_micromorphic_2019}
and in the framework of macroscopic strain-gradient approaches by
\cite{kouznetsova_multi-scale_2002,kouznetsova_multi-scale_2004,bacigalupo_second-order_2010,yvonnet_computational_2020}.
We refer to
\cite{forest_cosserat_1998,forest_generalized_2011}
for seminal treatments.  A Piola homogenisation is shown in \cite{delIsola2015} with applications on pantographic structures.

The present work is devoted to the \textit{multiscale computational homogenization of gradient-extended continua} and unites ingredients of the works of
\cite{kouznetsova_multi-scale_2002}
with respect to the gradient extensions at the homogenized \MK{macroscale}, of
\cite{miehe_computational_1999}
with regard to the algorithmic linearization of the macroscopic field equations, and of
\cite{cirak_subdivision_2000,hughes_isogeometric_2005}
with regard to spatial discretizations. In contrast to the contribution of
\cite{kouznetsova_multi-scale_2002},
which combines  a Cauchy continuum at the lower length scale \MK{(from now on denoted as microscale, representing the microstructure at each material point)} with a gradient-extended continuum at the larger \MK{macroscale}, we will take into account \textit{gradient-extended continua at both scales}.  \MK{Gradient-extended continua on the microscale can be taken into account, e.g.\ if embedded fibers on this scale are considered as continuum degenerated continua,  see \cite{khristenko2021,Schulte2020b} with analytical, numerical and experimental details on this prototypical example.}This endeavor poses additional challenges not only for the theoretical treatment, but also for the numerical implementation. The latter is due to the fact that the gradient extensions come along with the requirement of $C^1$-continuous approximations of independent fields at both scales. Such a requirement can be captured in an elegant way by employing \textit{isogeometric analysis} (IGA) in the sense of
\cite{cirak_subdivision_2000,hughes_isogeometric_2005}. For the application on fiber reinforced polymers, represented by second gradient materials, we refer to \cite{dittmann2020a}. A further algorithmic feature of the proposed implementation is due to the linearization of the macroscopic boundary value problem. Here, we employ the approach advocated by
\cite{miehe_computational_1999},
which was originally developed in the context of first-order homogenization. As we will see, the associated gradient extensions result in settings that remind of the linearized structures appearing in the coupled homogenization schemes considered by
\cite{schroder_two-scale_2012,keip_two-scale_2014,keip_multiscale_2016}.

\MK{As the present work proposes a computational multiscale method based on numerical discretizations involving isogeometric analysis at two scales, we denote it as IGA\textsuperscript{2}-method in analogy to the well-known FE\textsuperscript{2}-methods mentioned above. We refer to
\cite{schroder_numerical_2014}
for a review of FE\textsuperscript{2}-methods and to
\cite{matous_review_2017}
for a general overview of computational multiscale techniques. As already mentioned, the motivation behind using IGA instead of classical finite elements is due to the straightforward and elegant implementation of $C^1$-continuous independent fields. In case of classical FE methods, the contruction and implementation of higher-order element continuities is usually cumbersome. It could, for example, be realized by the use of Hermite shape functions, which however come with a complex algebraic structure and a high number of degrees of freedom, in particular in three spatial dimensions. Alternative FE approximations are given by mixed and non-conforming methods. While mixed methods can be implemented with standard $C^0$-type shape functions, they need to satisfy the inf-sup condition
(\cite{brezzi_mixed_1991}).
Non-conforming finite elements indeed allow for a more or less straightforward numerical implementation at a reasonable amount of degrees of freedom
(\cite{teichtmeister_phase_2017}),
still their finite-element function space is not a subspace of the solution space
(\cite{crouzeix_conforming_1973}).
In contrast to that, IGA-based schemes do not suffer from such limitations, but allow for an elegant implementation of higher-order continuities.%
\footnote{%
Alternative schemes with even $C^\infty$-continuous interpolations at the microscopic level have been proposed by
\cite{moulinec_numerical_1998}
and were recently implemented in the framework of so-called FE-FFT methods. As the name suggests, associated schemes combine macroscopic solvers based on finite elements with microscopic solvers based on spectral methods (Fast Fourier Transforms; FFT), see
\cite{spahn_multiscale_2014,kochmann_two-scale_2016,gokuzum_algorithmically_2018}.
}
As IGA-based multiscale methods have thus far been limited to homogeneous macroscopic problems
(\cite{alberdi_framework_2018,wang_optimal_2018}),
we believe that the here proposed IGA\textsuperscript{2}-method provides a useful and innovative framework for the modeling of higher-order continua across length scales.

The outline of the paper is as follows. In Section 2 we discuss fundamental concepts of the multiscale modeling of higher-gradient continua. In that consequence, suitable boundary conditions based on an energetically consistent scale transition are derived. In Section 3 we discuss the numerical implementation of the proposed scheme. Here, we put an emphasis on the consistent linearization of the macroscopic field equations and the IGA-based discretization of representative volume elements (RVE). In Section 4 we present a number of benchmark tests to demonstrate the performance and accuracy of the proposed multiscale technique. We close the paper with a summary and a conclusion in Section 5.}




%
%
%
%Materials with a significant microstructure, like composite materials or fiber-reinforced materials, are under development for many years. The mechanical response of this microstructure gives rise to additional higher-order terms of the considered continuum. The investigation of gradient materials started with the fundamental work of the Cosserat brothers \cite{cosserat1909} introducing coupled stresses over a hundred years ago. This has been generalized on second and third order theories in the work of Mindlin \cite{mindlin1964,mindlin1965} and Toupin \cite{toupin1964}. Different interpretations and notations are common nowadays for generalized continua; following Steinmann \cite{steinmann1997} we can introduce constrained and unconstrained higher-order contributions, e.g. coupled stresses as introduced by the Cosserat brothers are denoted as unconstrained micropolar continua.
%
%%Hence, we can make use of the concept of a director based theory for unconstrained, i.e.\ independent rotations, as introduced by Eringen \cite{eringen1964a,eringen1967a}, see also Hirschberger et al.\ \cite{steinmann2007} and Saanouni \& Hamed \cite{saanouni2013}. To be specific, a local director triad, representing the microcontinuum, is attached at every material point of the macrocontinuum. The triad consists in general of three deformable and independent directors, including the necessary information about the microstructure. A summary of the microcontinuum field theories is given in Eringen \cite{eringen1999}. Therein, a micromorphic continuum is called a microstretch continuum constraining the directors in shear (allowing only micro-rotations and micro-stretch), see Romeo \cite{Romeo2020} for the modeling of dielectric elastomers. Introducing rigid directors, we obtain a micropolar continuum, restricting the gradient contributions to rotations as often used for embedded fiber like structures, see Bauer et al.\ \cite{bauer2012}, Ramezani et al.\ \cite{ramezani2009} and Eringen \cite{eringen1966}.
%
%Mindlin \cite{mindlin1964,mindlin1965} laid the fundamentals for general higher-gradient theories in the 1960s, see also Germain \cite{germain1973b}, Toupin \cite{toupin1962,toupin1964}. The latter work of Mindlin \cite{mindlin1965} related an energy-density to the strain (second gradient) in linear elasticity, whereas Javili et al.\ \cite{steinmann2013} demonstrated a full non-linear framework on higher-order theories. A specific interpretation in terms of a director triad attached at every macroscopic point is given in Eringen \cite{eringen1964a,eringen1967a}, see also Hirschberger et al.\ \cite{steinmann2007} and Saanouni \& Hamed \cite{saanouni2013}. The correlation between the micromorphic and a second gradient theory is given in Kirchner \& Steinmann \cite{steinmann2005}.  The relationship between the microstructure and the macroscopic formulation as generalized continua is given in many publications, see among others Eringen \& Maugin \cite{eringen1990}, Maugin \& Metrikine \cite{maugin2010}, Forest \& Sievert \cite{forest2003}, Hirschberger et al.\ \cite{steinmann2007} and Saanouni \& Hamed \cite{saanouni2013}.  For a detailed view on the mathematical structure, see Javili et al.\ \cite{steinmann2013}, Kirchner \& Steinmann \cite{steinmann2005}, Aldakheel \cite{aldakheel2017a}, Neef \cite{neff2006}, Neff \& Jeong \cite{neff2009} and Yang et al.\ \cite{yang2002}.
%
%Higher-order gradient theories are widely used nowadays. We refer to dell'Isola et al.\ \cite{delIsola2015,hesch2019a} for applications on pantographic structures, whereas composites are addressed in Asmanoglo \& Menzel \cite{menzel2017a,menzel2017c}.  An extension of the latter formulation towards thermomechanical ductile fracture is proposed in Dittmann et al.\ \cite{dittmann2020a}. In Khristenko et al.\ \cite{khristenko2021} continuum degenerated beam formulations have been immersed within a 3D matrix material. A static condensation procedure leads to an anisotropic second gradient formulation for the bending and torsion of the beam within the matrix material.
%
%Attached unit cells or representative volume elements ($\RVE$) are used in Keip et al.\ \cite{keip2014} and Schr\"oder \& Keip \cite{keip2012} for electro-mechanically coupled boundary value problems. Here, first gradient theories are applied for the displacement and the electric potential. Furthermore, a two-scale homogenization approach is implemented with the FE$^2$-method using a consistent linearization of the macroscopic stresses. In Kouznetsova \cite{kouznetsovaPHD2002} and Kouznetsova et al. \cite{kouznetsova2002} a homogenization of a microscopic first order Cauchy continuum to a second order macroscopic continuum is presented.
%
%To deal with higher-order continuity requirements,  isogeometrical analysis (IGA) has become popular in recent years. IGA employs the same NURBS basis functions for the geometric design as well as for the analysis and was introduced in \cite{hughes2005}. It allows for the construction of finite element basis functions with adjustable continuity across the element boundaries, in contrast to classical Lagrangian basis functions, which are always \(C^0\) continuous at the element boundaries. This enables the numerical treatment of higher-order partial differential equations, e.g.\ for Cahn-Hilliard or Cahn-Hilliard like formulations \cite{gomez2008,hesch2016b,schuss2018a}, in fracture mechanics \cite{borden2014,dittmann2017b,dittmann2018,hesch2016a}, in structural mechanics, e.g.\ in \cite{benson2010,benson2011,dornisch2013,dornisch2016,Echter2013,kiendl2009,reali2015} and for generalized continua \cite{Fischer2011}. 
%
%In this work, we generalize the formulation of Kouznetsova and Keip et al.\ on higher-order material models. We allow for second and third order macroscopic continua, with first and second order continua within the microstructure, represented by a suitable $\RVE$ for the two-scale homogenization.  To take the higher-order continua into account, an IGA discretization is applied with sufficient regularity for the solution of the gradient contributions. The same IGA approach is applied on the macroscopic boundary value problem, i.e.\ we can make use of the terminus IGA$^2$-method.  To obtain the macroscopic stresses and hyperstresses,  we solve at each material point of the macroscopic material with given strains the microscopic $\RVE$. Afterwards, a homogenization procedure using a volumetric averaging is performed on the required quantities. To solve the macroscopic boundary value problem, a consistent linearization is required, introduced here as well for general higher-order theories.
%
%The paper is structured as follows: The macroscopic boundary value problem for the second gradient continua is introduced in Section \ref{sec:preliminaries} to illustrate the general setting. The microscopic boundary value problem as well as the homogenization using second or third gradient continua on the macroscale is presented in Section \ref{sec:micro}. In Section \ref{sec:discretization} we discretize both boundary value problems and linearize consistently the macroscopic stresses. Numerical examples are presented in Section \ref{sec:numerics} and conclusions are drawn in Section  \ref{sec:conclusions}.



==> sections/sec_homogenization_CH.tex <==
\subsection{Macroscopic boundary value problem}
We start with a short summary of the second-gradient macroscopic continuum. Therefore, we introduce a reference configuration $\Omega_0\subset \mathbb{R}^3$ with boundary $\partial\Omega_0$ and outward unit normal $\ma{N}$ and a current configuration $\Omega\subset \mathbb{R}^3$  with boundary $\partial\Omega$ and outward unit normal $\ma{n}$. The deformation mapping $\ma{\varphi}:\Omega_0\rightarrow\mathbb{R}^3$ relates the reference and actual configuration to each other, $\Omega=\ma{\varphi}(\Omega_0)$. Furthermore, the vectors to the material points $P$ are labeled by $\ma{X}\in\Omega_0$. In the actual configuration, these points $p$ are given by $\ma{x}=\ma{\varphi}(\ma{X})$, see Figure \ref{fig:Ref_Act}.

\begin{figure}[htb]
	\centering
	\begin{minipage}[top]{0.6\textwidth}
	\psfrag{x}{$\ma{x}$}
	\psfrag{X}{$\ma{X}$}
	\psfrag{x1}{$\vec{e}_1$}
	\psfrag{x2}{$\vec{e}_2$}
	\psfrag{x3}{$\vec{e}_3$}
	\psfrag{p}{$p$}
	\psfrag{P}{$P$}
	\psfrag{B0}{$\Omega_0$}
	\psfrag{Bt}{$\Omega$}
	\psfrag{dB0}{$\partial\Omega_0$}
	\psfrag{dBt}{$\partial\Omega$}
		\includegraphics[width=\textwidth]{figures/Ref_Act.eps}
	\end{minipage}
	\caption{Reference and actual configuration.}
	\label{fig:Ref_Act}
\end{figure}
The deformation gradient $\ma{F}:\Omega_0\rightarrow\mathbb{R}^{3\times3}$ and the third order tensor $\trima{F}:\Omega_0\rightarrow\mathbb{R}^{3\times3\times3}$ as the first and second derivative of the mapping $\ma{\varphi}(\ma{X})$:
\begin{equation}
\ma{F}=\bar\nabla\ma{\varphi}\qquad\text{and}\qquad\trima{F}=\bar\nabla^2\ma{\varphi}\,,
\end{equation}
where $\bar\nabla$ refers to the gradient with respect to $\bar{\vec{X}}$.  Following [???],  we postulate the virtual work of the internal contributions as follows 
\begin{equation}\label{virt_int_work}
\delta\Pi^{int}=\intRVE\ma{P}:\delta\ma{F}+\trima{P}\,\vdots\,\delta\trima{F}\,\d V\,,
\end{equation}
where $\ma{P}$ denotes the macroscopic two-field first Piola-Kirchhoff stress tensor and $\trima{P}$ the macroscopic two-field third-order stress tensor, conjugate to $\trima{F}$.  Here,
\begin{equation}
\delta\ma{F}=\bar\nabla\delta\ma{\varphi}\qquad\text{and}\qquad\delta\trima{F}=\bar\nabla^2\delta\ma{\varphi}\,,
\end{equation}
where the space of virtual or admissible test functions is given by
\begin{equation}
\mathbb{V} = \{\delta\vec{\varphi}\in \mathcal{H}^2(\Omega) | \delta\vec{\varphi} = \vec{0},\,\nabla\vec{\varphi}\cdot\bar{\vec{N}} = \vec{0} \;\text{on}\;\Gamma^{\varphi}\},
\end{equation}
The external contributions to the virtual work are given by
\begin{equation}
\delta\Pi^{ext}= \intRVE \ma{B}_{ext}\cdot\delta\ma{\varphi}\,\d V +
\int\limits_{\Gamma^{\sigma}} \ma{T}_{ext}\cdot\delta\ma{\varphi}\, \d A + \int\limits_{\Gamma^r}\ma{M}_{ext}:\nabla\delta\ma{\varphi}\,\d A
\end{equation}
with the common body force per unit volume $\ma{B}_{ext}$, the traction forces $\ma{T}_{ext}$ on boundary $\Gamma^{\sigma}$ and the double force traction $\ma{M}_{ext}$ on boundary $\Gamma^{r}$, see Figure \ref{fig:Macro_RVE}.

\begin{figure}[htb]
	\centering
	\begin{minipage}[top]{0.8\textwidth}
	\psfrag{barx}{$\ma{X}\in\Omega_0$}
	\psfrag{x}{$\mi{x}$}
	\psfrag{x1}{$\vec{e}_1$}
	\psfrag{x2}{$\vec{e}_2$}
	\psfrag{x3}{$\vec{e}_3$}
	\psfrag{Bu}{$\Gamma^\varphi$}
	\psfrag{Br}{$\Gamma^r$}
	\psfrag{Bs}{$\Gamma^\sigma$}
	\psfrag{micro}{$\RVE$}
	\psfrag{di}{$\vec{d}_I$}
	\psfrag{x}{$\mi{x}$}
	\psfrag{Rd}[][]{\begin{minipage}{4cm}\begin{center}\begin{footnotesize}
 $\RVE$ driven by\\ $\ma{F},\,\trima{F}$	\end{footnotesize}\end{center}\end{minipage}}
	\psfrag{cons}[][]{\begin{minipage}{4cm}\begin{center}\begin{footnotesize}
constitutive quantities\\ $\ma{P},\,\trima{P},\Delta\ma{P},\,\Delta\trima{P}$	\end{footnotesize}\end{center}\end{minipage}}
	\includegraphics[width=\textwidth]{figures/Macro_RVE.eps}
	\end{minipage}
	\caption{Micro-macro transition of mechanical boundary value problem, left: boundary decomposition of macro continuum in a Dirichlet boundary $\Gamma^\varphi$ and Neumann boundaries $\Gamma^{\sigma}$, $\Gamma^{r}$ of the traction force and double traction force, right: $\RVE$ as defined for every macroscopic point.}
	\label{fig:Macro_RVE}
\end{figure}

These can be related to the internal contributions (\ref{virt_int_work}) by applying partial integration and the Gaussian integral theorem, see Javili et al.\ \cite{steinmann2013}:
\begin{equation}\label{int_ext_cont}
\begin{aligned}
\ma{T}_{ext}&=(\ma{P}-\bar{\nabla}\cdot\trima{P})\,\ma{N}\,,\\
\ma{M}_{ext}&=\trima{P}\,\ma{N}\,.
\end{aligned}
\end{equation}
Note, that the last equation can be decomposed in tangential and normal components, see Neff et al. [???] for details. Taking the balance equations
\begin{equation}\label{eq:macro_strong}
\bar{\nabla}\cdot(\ma{P}-\bar{\nabla}\cdot\trima{P}) + \ma{B}_{ext}=\vec{0}\,.\\
\end{equation}
into account,  completes the set of equations for the strong form of the second gradient boundary value problem.

\subsection{Microscopic boundary value problem}\label{sec:micro}
In every material point $P$, we assume the existence of a representative finite domain $\RVE$ containing the information on the inhomogeneous microscopic continuum. To be specific, we assume the existence of a second gradient material in the domain $\RVE$; this general approach for the homogenisation from a second gradient microcontinuum towards a second gradient macrocontinuum allows us to demonstrate that the formulation proposed by Kouznetsova et al.\ \cite{Kouznetsova2004b} is a special case of the methodology presented next.

We start with the mapping for the microscopic relative position of the material points $\mi{x}=\mi{\varphi}(\mi{X})$:
\begin{equation}
\mi{\varphi}(\mi{X})= \ma{F}\,\mi{X}+\frac{1}{2}\,\trima{F}:(\mi{X}\otimes\mi{X})+\fluc{w}\,.
\end{equation}
%This is a Taylor series expansion of the well-known linear mapping in classical continuum mechanics, which leads to a nonlinear mapping of $\mi{X}\rightarrow\mi{x}$. 
Here, $\fluc{w}$ describes the unknown microcroscopic fluctuation field, which includes all higher-order terms of the Taylor series expansion, see Kouznetsova et al.\ \cite{Kouznetsova2004b}.  
Analogous to the macroscopic quantities, we obtains the microscopic deformation tensor $\mi{F}$ and the third-order tensor $\trimi{F}$: 
\begin{equation}
\mi{F}=\nabla\mi{\varphi}\qquad\text{and}\qquad\trimi{F}=\nabla\mi{F}=\nabla^2\mi{\varphi}\,.
\end{equation}
We note that the macroscopic values are exactly the volume averages of the microscopic values.  Hence, we can write
\begin{equation}\label{restrictions}
\frac{1}{V}\,\intRVE \nabla\fluc{w}\,\d V=\vec{0}\qquad\text{and}\qquad\frac{1}{V}\,\intRVE \nabla^2\fluc{w}\,\d V=\trimi{0}\,.
\end{equation}
The averaged microscopic deformations over the volume of the $\RVE$ can be connected to the macroscopic counterparts $\ma{F}$ and $\trima{F}$ via
\begin{equation}\label{eq:mi_ma_F}
\frac{1}{V}\,\intRVE\mi{F}\,\d V=\frac{1}{V}\,\intRVE\,\left(\ma{F}+\trima{F}\,\vec{X}+\fluc{F}\right)\,\d V=\ma{F}
\end{equation}
and
\begin{equation}\label{eq:mi_ma_triF}
\frac{1}{V}\,\intRVE\trimi{F}\,\d V=\frac{1}{V}\,\intRVE\,\left(\trima{F}+\trifluc{F}\right)\,\d V=\trima{F}
\end{equation}
using $\intRVE\vec{X}\d V=\vec{0}$, which is valid if the coordinate system is in the center of the $\RVE$. Furthermore, $\fluc{F}=\nabla\fluc{w}$ and $\trifluc{F}=\nabla^2\fluc{w}$ are the first and second gradients of the fluctuation field, which have to fulfil \eqref{restrictions}. The local balance equations of the microscopic second gradient continuum is given analogously to (\ref{eq:macro_strong}) by:
\begin{equation}\label{eq:micro_strong}
\nabla\cdot\left[\mi{P} - \nabla\cdot\trimi{P}\right]=\vec{0}\,,
\end{equation}
where $\mi{P}:=\partial_{\mi{F}}\Psi(\mi{F},\trimi{F})$ and $\trimi{P}:=\partial_{\trimi{F}}\Psi(\mi{F},\trimi{F})$ are defined by the derivatives of the Helmholz energy functional $\Psi$. 

%For the complete description of the microscopic boundary value problem, appropriate boundary conditions on the boundary $\partial\RVE$ and some constraints for the whole $\RVE$ will be defined. Therefore, we apply a homogeneity condition, given by the Hill-Mandel criteria. 

The homogeneity condition as given by the Hill-Mandel criteria states that the virtual work applied to the system in the material point $P$ is equal to the virtual work in the domain $\RVE$, hence
\begin{equation}\label{eq:Hill_Mandel}
\frac{1}{V}\intRVE\bigl(\mi{P}:\nabla\delta\mi{\varphi}+ \mathfrak{P}\,\vdots\,\nabla^2\delta\mi{\varphi}\bigr)\d V =\ma{P}:\delta\ma{F} +\trima{P}\,\vdots\,\delta\trima{F}\,.
\end{equation}
The left side of the Hill Mandel criteria can be rewritten as follows
\begin{equation}
\frac{1}{V}\,\intRVE\mi{P}\,\d V:\delta\ma{F}+\frac{1}{V}\,\intRVE\bigl(\trimi{P}+\mi{P}\otimes\mi{X}\bigr)\,\d V\,\vdots\,\delta\trima{F} =\ma{P}:\delta\ma{F} +\trima{P}\,\vdots\,\delta\trima{F}\,,
\end{equation}
see Appendix \ref{app:Deriv_stresses}. Comparing the left and right side of the last equation, yields 
\begin{equation}\label{eq:mi_ma_stresses}
\ma{P}=\frac{1}{V}\intRVE\mi{P}\,\d V\qquad\text{and}\qquad
\trima{P}=\underbrace{\frac{1}{V}\intRVE\trimi{P}\, \d V}_{\trima{P}^{\trimi{P}}}+\underbrace{\frac{1}{V}\intRVE\mi{P}\otimes\mi{X}\, \d V}_{\trima{P}^{\mi{P}}}\,.  
\end{equation}
Note that the macroscopic third-order stress tensor $\trima{P}$ is split into $\trima{P}^{\trimi{P}}$, which is a volume average of the microscopic third-order stress tensor $\trimi{P}$, and $\trima{P}^{\mi{P}}$, which is given by the volume average of the first moment of the microscopic stresses $\mi{P}$. Assuming a first gradient material within the $\RVE$ removes the macroscopic hyperstress $\trima{P}^{\trimi{P}}$ and we obtain the formulation provided by Kouznetsova et al.\ \cite{Kouznetsova2004b}. For appropriate boundary conditions, the Hill-Mandel criteria can be rewritten as:
\begin{equation}\label{eq:deriv_boundary1}
\frac{1}{V}\intRVE\left[\ma{P}-\mi{P}\right]:[\delta\ma{F}+\delta\trima{F}\cdot\vec{X}-\delta\mi{F}]+\left[\trima{P}^{\trimi{P}}-\trimi{P}\right]\,\vdots\,\left[\delta\trima{F}-\delta\trimi{F}\right]\,\d V=0\,,
\end{equation}
see Appendix \ref{app:rew_Hill_Mandel}. Obviously, the simplest assumption for all points of the microscopic scale, that fullfils the last equation is given by postulating the constraints $\ma{P}:=\mi{P}$ or $\delta\ma{F}+\delta\trima{F}\cdot\vec{X}:=\delta\mi{F}$ and additionally $\trima{P}^\trimi{P}:=\trimi{P}$ or $\delta\trima{F}:=\delta\trimi{F}$, compare Keip et al.\ \cite{keip2014}. An alternative expression of (\ref{eq:deriv_boundary1}) yields suitable and more general boundary conditions:
\begin{equation}\label{eq:deriv_boundary2}
\begin{aligned}
&\frac{1}{V}\dintRVE\left(\left[\trima{P}_1-\trimi{P}\right]\,\mi{N}\right):\left[\delta\ma{F}+\delta\trima{F}\cdot\mi{X}-\delta\mi{F}\right]\,\d A\\
+&\frac{1}{V}\dintRVE\left(\left[\ma{P}-\left(\mi{P}-\nabla\cdot\trimi{P}\right)\right]\,\mi{N}\right)\cdot\left[\delta\ma{F}\,\mi{X}+\frac{1}{2}\,\delta\trima{F}:(\mi{X}\otimes\mi{X})-\delta\mi{\varphi}\right]\,\d A=0\,,\end{aligned} 
\end{equation}
see Appendix \ref{app:bc_Hill_Mandel} for further information.
%Furthermore, we get the restrictions for the fluctuation:
%\begin{equation}
%\frac{1}{V}\,\intRVE\nabla\fluc{w}\,\d V=\vec{0}\qquad\text{and}\qquad\frac{1}{V}\,\intRVE\nabla^2\fluc{w}\,\d V=\vec{0}\,,
%\end{equation}
%since the macroscopic magnitudes have to be independent of the fluctuation.

\begin{remark}
Third gradient medium: Hyperstress $\trima{G}$ connected to $\ma{P}\otimes\vec{X}\otimes\vec{X} + \trima{P}\otimes\vec{X}$?
\end{remark}



==> sections/sec_homogenization_MK.tex <==
\subsection{Macroscopic boundary value problem}
We start with a short summary of the second-gradient macroscopic continuum. Therefore, we introduce a reference configuration $\Omega_0\subset \mathbb{R}^3$ with boundary $\partial\Omega_0$ and outward unit normal $\ma{N}$ and a current configuration $\Omega\subset \mathbb{R}^3$  with boundary $\partial\Omega$ and outward unit normal $\ma{n}$. The deformation mapping $\ma{\varphi}:\Omega_0\rightarrow\mathbb{R}^3$ relates the reference and actual configuration to each other, $\Omega=\ma{\varphi}(\Omega_0)$. Furthermore, the vectors to the material points $P$ are labeled by $\ma{X}\in\Omega_0$. In the actual configuration, these points $p$ are given by $\ma{x}=\ma{\varphi}(\ma{X})$, see Figure \ref{fig:Ref_Act}.

\begin{figure}[htb]
	\centering
	\begin{minipage}[top]{0.6\textwidth}
	\psfrag{x}{$\ma{x}$}
	\psfrag{X}{$\ma{X}$}
	\psfrag{x1}{$\vec{e}_1$}
	\psfrag{x2}{$\vec{e}_2$}
	\psfrag{x3}{$\vec{e}_3$}
	\psfrag{p}{$p$}
	\psfrag{P}{$P$}
	\psfrag{B0}{$\Omega_0$}
	\psfrag{Bt}{$\Omega$}
	\psfrag{dB0}{$\partial\Omega_0$}
	\psfrag{dBt}{$\partial\Omega$}
		\includegraphics[width=\textwidth]{figures/Ref_Act.eps}
	\end{minipage}
	\caption{Reference and actual configuration.}
	\label{fig:Ref_Act}
\end{figure}
The deformation gradient $\ma{F}:\Omega_0\rightarrow\mathbb{R}^{3\times3}$ and the third order tensor $\trima{F}:\Omega_0\rightarrow\mathbb{R}^{3\times3\times3}$ as the first and second derivative of the mapping $\ma{\varphi}(\ma{X})$:
\begin{equation}
\ma{F}=\bar\nabla\ma{\varphi}\qquad\text{and}\qquad\trima{F}=\bar\nabla\ma{F} = \bar\nabla^2\ma{\varphi}\,.
\end{equation}
Thus, the virtual work of the internal contributions is derived by the two independent variables $\ma{F}$ and $\trima{F}$:
\begin{equation}\label{virt_int_work}
\delta\Pi^{int}=\int\limits_{\Omega_0}\ma{P}:\delta\ma{F}+\trima{P}\,\vdots\,\delta\trima{F}\,\d V\,,
\end{equation}
where $\ma{P}$ denotes the macroscopic Piola-Kirchhoff stress tensor and $\trima{P}$ is the macroscopic third-order stress tensor. These two stresses are not derived, as in a classical continuum, by the free energy function $\Psi$. The constitutive law is given in the microscopic continuum (see section \ref{sec:micro}) and is transferred by a homogenization technique to the macroscopic continuum. Nevertheless, the internal contributions stand opposite the external contributions as before, which are:
\begin{equation}
\delta\Pi^{ext}= \intRVE \ma{B}_{ext}\cdot\delta\ma{\varphi}\,\d V +
\int\limits_{\Gamma^{\sigma}} \ma{T}_{ext}\cdot\delta\ma{\varphi}\, \d A + \int\limits_{\Gamma^r}(\ma{R}_{ext}\otimes\ma{N}):\nabla\delta\ma{\varphi}\,\d A
\end{equation}
with the common body force per unit volume $\ma{B}_{ext}$, the traction forces $\ma{T}_{ext}$ on boundary $\Gamma^{\sigma}$ and the double stress traction $\ma{R}_{ext}$ on boundary $\Gamma^{r}$, see Figure \ref{fig:Macro_RVE}.

\begin{figure}[htb]
	\centering
	\begin{minipage}[top]{0.8\textwidth}
	\psfrag{barx}{$\ma{x}\in\Omega$}
	\psfrag{x}{$\mi{x}$}
	\psfrag{x1}{$\vec{e}_1$}
	\psfrag{x2}{$\vec{e}_2$}
	\psfrag{x3}{$\vec{e}_3$}
	\psfrag{Bu}{$\Gamma^\varphi$}
	\psfrag{Br}{$\Gamma^r$}
	\psfrag{Bs}{$\Gamma^\sigma$}
	\psfrag{micro}{$\RVE$}
	\psfrag{di}{$\vec{d}_I$}
	\psfrag{x}{$\mi{x}$}
	\psfrag{Rd}[][]{\begin{minipage}{4cm}\begin{center}\begin{footnotesize}
 $\RVE$ driven by\\ $\ma{F},\,\trima{F}$	\end{footnotesize}\end{center}\end{minipage}}
	\psfrag{cons}[][]{\begin{minipage}{4cm}\begin{center}\begin{footnotesize}
constitutive quantities\\ $\ma{P},\,\trima{P},\Delta\ma{P},\,\Delta\trima{P}$	\end{footnotesize}\end{center}\end{minipage}}
	\includegraphics[width=\textwidth]{figures/Macro_RVE.eps}
	\end{minipage}
	\caption{Micro-macro transition of mechanical boundary value problem, left: boundary decomposition of macro continuum in a Dirichlet boundary $\Gamma^\varphi$ and Neumann boundaries $\Gamma^{\sigma}$, $\Gamma^{r}$ of the traction force and double traction force, right: attached $\RVE$ for every macroscopic point $a$.}
	\label{fig:Macro_RVE}
\end{figure}

These can be related to the internal contributions (\ref{virt_int_work}) by applying partial integration and the Gaussian integral theorem, see Javili et al.\ \cite{steinmann2013}:
\begin{equation}\label{int_ext_cont}
\begin{aligned}
\ma{B}_{ext} &= -\bar{\nabla}\cdot(\ma{P}-\bar{\nabla}\cdot\trima{P})\,,\\
\ma{T}_{ext}&=(\ma{P}-\bar{\nabla}\cdot\trima{P})\,\ma{N}+(\bar{\nabla}_{\|}\cdot\ma{N})\,(\trima{P}\,\ma{N})\,\ma{N}-\bar{\nabla}_{\|}\cdot(\trima{P}\,\ma{N})\,,\\
\ma{R}_{ext}&=(\trima{P}\,\ma{N})\,\ma{N}\,.
\end{aligned}
\end{equation}
Assuming a smooth surface, we neglect line integrals. Furthermore, we ignore body forces $\ma{B}_{ext}=\vec{0}$, so that the strong boundary value problem of (\ref{int_ext_cont})$_1$ for the macrosopic continuum is given by:
\begin{equation}\label{eq:macro_strong}
\bar{\nabla}\cdot(\ma{P}-\bar{\nabla}\cdot\trima{P})=\vec{0}\,.\\
\end{equation}

\subsection{Microscopic boundary value problem}\label{sec:micro}
In every macroscopic finite point $P$ and $p$, respectively, we attach a representative volume element ($\RVE$) to describe the microscopic continuum that contains the constitutive law. We start with the description of the mapping for the microscopic relative position of the material points $\mi{x}=\mi{\varphi}(\mi{X})$:
\begin{equation}\label{eq:mi_kinematic}
\mi{\varphi}(\mi{X})= \ma{F}\,\mi{X}+\frac{1}{2}\,\trima{F}:(\mi{X}\otimes\mi{X})+\fluc{w}\,.
\end{equation}
This is a Taylor series expansion of the well-known linear mapping in classical continuum mechanics, which leads to a nonlinear mapping of $\mi{X}\rightarrow\mi{x}$. Here, $\fluc{w}$ describes the unknown microcroscopic fluctuation field, which includes all higher-order terms of the Taylor series, see Kouznetsova et al.\ \cite{Kouznetsova2004b}. Analogous to the macroscopic quantities, one obtains the microscopic deformation tensor $\mi{F}$ and the third-order tensor $\trimi{F}$: 
\begin{equation}
\mi{F}=\nabla\mi{\varphi}\qquad\text{and}\qquad\trimi{F}=\nabla\mi{F}=\nabla^2\mi{\varphi}\,.
\end{equation}
The averaged microscopic deformations over the volume of the $\RVE$ can be connected to the macroscopic counterparts $\ma{F}$ and $\trima{F}$ in the point $p$:
\begin{equation}\label{eq:mi_ma_F}
\frac{1}{V}\,\intRVE\mi{F}\,\d V=\frac{1}{V}\,\intRVE\,\left(\ma{F}+\trima{F}\,\vec{X}+\fluc{F}\right)\,\d V=\ma{F}
\end{equation}
and
\begin{equation}\label{eq:mi_ma_triF}
\frac{1}{V}\,\intRVE\trimi{F}\,\d V=\frac{1}{V}\,\intRVE\,\left(\trima{F}+\trifluc{F}\right)\,\d V=\trima{F}
\end{equation}
using that $\frac{1}{V}\,\intRVE\vec{X}\d V=\vec{0}$, if the coordinate system is in the center of the $\RVE$, and that the macroscopic quantities are independent of the $\RVE$. Furthermore, $\fluc{F}=\nabla\fluc{w}$ and $\trifluc{F}=\nabla^2\fluc{w}$ are the gradients of the fluctuation field and we enforce the equality of the macroscopic gradients to the average of the microscopic counterparts. This yields the following restrictions for (\ref{eq:mi_ma_F}) and (\ref{eq:mi_ma_triF}):
\begin{equation}\label{eq:restr_kinematic}
\frac{1}{V}\,\intRVE \nabla\fluc{w}\,\d V=\vec{0}\qquad\text{and}\qquad\frac{1}{V}\,\intRVE \nabla^2\fluc{w}\,\d V=\trimi{0}\,.
\end{equation}

The strong form of the microscopic second gradient continuum is given analogously to (\ref{eq:macro_strong}) by:
\begin{equation}\label{eq:micro_strong}
\nabla\cdot\left[\mi{P} - \nabla\cdot\trimi{P}\right]=\vec{0}\,,
\end{equation}
where $\mi{P}:=\partial_{\mi{F}}\Psi(\mi{F},\trimi{F})$ and $\trimi{P}:=\partial_{\trimi{F}}\Psi(\mi{F},\trimi{F})$ are defined by the derivatives of the free energy function $\Psi$. For the complete description of the microscopic boundary value problem, appropriate boundary conditions on the boundary $\partial\RVE$ and some constraints for the whole $\RVE$ will be defined. Therefore, we apply a homogeneity condition, given by the Hill-Mandel criteria. 

The idea of the Hill-Mandel criteria is, that the virtual works of the macro system in the point are equal to the averaged virtual works in the micro system:
\begin{equation}\label{eq:Hill_Mandel}
\frac{1}{V}\intRVE\bigl(\mi{P}:\nabla\delta\mi{\varphi}+ \mathfrak{P}\,\vdots\,\nabla^2\delta\mi{\varphi}\bigr)\d V =\ma{P}:\delta\ma{F} +\trima{P}\,\vdots\,\delta\trima{F}\,.
\end{equation}
The left side of the Hill Mandel criteria can be rewritten, see Appendix \ref{app:Deriv_stresses}, such that the whole criteria is given by:
\begin{equation}
\frac{1}{V}\,\intRVE\mi{P}\,\d V:\delta\ma{F}+\frac{1}{V}\,\intRVE\bigl(\trimi{P}+\mi{P}\otimes\mi{X}\bigr)\,\d V\,\vdots\,\delta\trima{F} =\ma{P}:\delta\ma{F} +\trima{P}\,\vdots\,\delta\trima{F}\,.
\end{equation}
Comparing the left and right side of the last equation, yields the macroscopic stresses
\begin{equation}\label{eq:mi_ma_stresses}
\ma{P}=\frac{1}{V}\intRVE\mi{P}\,\d V\qquad\text{and}\qquad
\trima{P}=\underbrace{\frac{1}{V}\intRVE\trimi{P}\, \d V}_{\trima{P}^{\trimi{P}}}+\underbrace{\frac{1}{V}\intRVE\mi{P}\otimes\mi{X}\, \d V}_{\trima{P}^{\mi{P}}}\,.  
\end{equation}
It is obvious, that the macroscopic stresses $\ma{P}$ are given by the volume average of the microscopic stresses $\mi{P}$. The macroscopic third-order stress tensor $\trima{P}$ is split into $\trima{P}^{\trimi{P}}$, which is a volume average of the microscopic third-order stress tensor $\trimi{P}$, and $\trima{P}^{\mi{P}}$, which is given by the volume average of the first moment of the microscopic stresses $\mi{P}$.

For appropriate boundary conditions, the Hill-Mandel criteria is rewritten as:
\begin{equation}\label{eq:deriv_boundary1}
\frac{1}{V}\intRVE\left[\ma{P}-\mi{P}\right]:[\delta\ma{F}+\delta\trima{F}\cdot\vec{X}-\delta\mi{F}]+\left[\trima{P}^{\trimi{P}}-\trimi{P}\right]\,\vdots\,\left[\delta\trima{F}-\delta\trimi{F}\right]\,\d V=0\,,
\end{equation}
see Appendix \ref{app:rew_Hill_Mandel}. Obviously, the simplest assumption for all points of the microscopic scale, that fullfils the last equation is given by postulating the constraints $\ma{P}:=\mi{P}$ or $\delta\ma{F}+\delta\trima{F}\,\vec{X}:=\delta\mi{F}$ and additionally $\trima{P}^\trimi{P}:=\trimi{P}$ or $\delta\trima{F}:=\delta\trimi{F}$, compare Keip et al.\ \cite{keip2014}. An alternative expression of (\ref{eq:deriv_boundary1}) yields suitable and more general boundary conditions:
\begin{equation}\label{eq:deriv_boundary2}
\begin{aligned}
&\frac{1}{V}\dintRVE\left(\left[\trima{P}^\trimi{P}-\trimi{P}\right]\,\mi{N}\right):\left[\delta\ma{F}+\delta\trima{F}\,\mi{X}-\delta\mi{F}\right]\,\d A\\
+&\frac{1}{V}\dintRVE\left(\left[\ma{P}-\left(\mi{P}-\nabla\cdot\trimi{P}\right)\right]\,\mi{N}\right)\cdot\left[\delta\ma{F}\,\mi{X}+\frac{1}{2}\,\delta\trima{F}:(\mi{X}\otimes\mi{X})-\delta\mi{\varphi}\right]\,\d A=0\,,\end{aligned} 
\end{equation}
see Appendix \ref{app:bc_Hill_Mandel} for further information. Thus the Dirichlet and Neumann boundary conditions are:
\begin{equation}
\begin{aligned}
\delta\ma{F}\,\mi{X}+\frac{1}{2}\,\delta\trima{F}:(\mi{X}\otimes\mi{X})-\delta\mi{\varphi}&=\vec{0}\,,\qquad&\qquad \ma{P}\,\mi{N}&=\mi{T}_{ext}\\
\delta\ma{F}+\delta\trima{F}\,\mi{X}-\delta\mi{F}&=\vec{0}\,,\qquad&\qquad\trima{P}^\trimi{P}\,\mi{N}&=\mi{R}_{ext}
\end{aligned}
\end{equation}
A comparison of the boundary conditions with (\ref{eq:var_mi_kinematic}) provides the following relationship for these conditions, $\delta\fluc{w}=\vec{0}$ and $\delta\nabla\fluc{w}=\vec{0}$. Furthermore, the Neumann boundaries are given by the microscopic tractions $\mi{T}_{ext}=\left(\mi{P}-\nabla\cdot\trimi{P}\right)\,\mi{N}$ and double tractions $\mi{R}_{ext}=\trimi{P}\,\mi{N}$. Using periodic boundary conditions, see Figure (\ref{fig:periodic}),
\begin{equation}
\begin{aligned}
\fluc{w}^+(\mi{x}^+)&=\fluc{w}^-(\mi{x}^-)\,,\qquad&\qquad\mi{T}^+_{ext}(\mi{x}^+)&=-\mi{T}^-_{ext}(\mi{x}^-)\,,\\
\nabla\fluc{w}^+(\mi{x}^+)&=\nabla\fluc{w}^-(\mi{x}^-)\,,&\mi{R}^+_{ext}(\mi{x}^+)&=-\mi{R}^-_{ext}(\mi{x}^-)\,.
\end{aligned}
\end{equation}
we can satisfy the Hill-Mandel criteria (\ref{eq:Hill_Mandel}). The restrictions for the stresses (\ref{eq:restr_stresses}) of the Hil-Mandel criteria as well as the restrictions for the kinematic (\ref{eq:restr_kinematic}) are fulfilled with periodic boundary conditions. 

\begin{figure}[htb]
	\centering
	\begin{minipage}[top]{0.6\textwidth}
	\psfrag{a}{$\partial\RVE$}
	\psfrag{b}{$\partial\RVE$}
	\psfrag{phi}{$\mi{\varphi}(\mi{X})$}
	\psfrag{x}{$\mi{x}$}
	\psfrag{X}{$\mi{X}$}
	\psfrag{np}{$\mi{N}^+$}
	\psfrag{nm}{$\mi{N}^-$}
	\psfrag{+}{$+$}
	\psfrag{-}{$-$}
	\includegraphics[width=\textwidth]{figures/periodic.eps}
	\end{minipage}
	\caption{Microscopic boundary value problem, periodic boundary conditions on $\partial\RVE$, here only displayed for top and bottom for better understanding.}
	\label{fig:periodic}
\end{figure}


\textbf{Remark:}


==> sections/sec_numerics_FSchmidt.tex <==
% Energies first gradient material, order 2, [4 8 16] Elements
% sorting: 4-diri & 4-peri & 8-diri & 8-peri & 16-diri & 16-peri
% \pA = abs(E(4-diri)-E(4-diri)) / E(4-diri)
% \pB = abs(E(4-diri)-E(4-peri)) / E(4-diri)

\renewcommand{\pA}{$0$}
\renewcommand{\pB}{$0.00e+00$}
\renewcommand{\pC}{$1.07\mathrm{E}{-}15$}
\renewcommand{\pD}{$1.07\mathrm{E}{-}15$}
\renewcommand{\pE}{$8.77\mathrm{E}{-}15$}
\renewcommand{\pF}{$8.77\mathrm{E}{-}15$}
\renewcommand{\pG}{$0.00e+00$}
\renewcommand{\pH}{$0$}
\renewcommand{\pI}{$1.07\mathrm{E}{-}15$}
\renewcommand{\pJ}{$1.07\mathrm{E}{-}15$}
\renewcommand{\pK}{$8.77\mathrm{E}{-}15$}
\renewcommand{\pL}{$8.77\mathrm{E}{-}15$}
\renewcommand{\pM}{$1.07\mathrm{E}{-}15$}
\renewcommand{\pN}{$1.07\mathrm{E}{-}15$}
\renewcommand{\pO}{$0$}
\renewcommand{\pP}{$0.00e+00$}
\renewcommand{\pQ}{$7.70\mathrm{E}{-}15$}
\renewcommand{\pR}{$7.70\mathrm{E}{-}15$}
\renewcommand{\pS}{$1.07\mathrm{E}{-}15$}
\renewcommand{\pT}{$1.07\mathrm{E}{-}15$}
\renewcommand{\pU}{$0.00e+00$}
\renewcommand{\pV}{$0$}
\renewcommand{\pW}{$7.70\mathrm{E}{-}15$}
\renewcommand{\pX}{$7.70\mathrm{E}{-}15$}
\renewcommand{\pY}{$8.77\mathrm{E}{-}15$}
\renewcommand{\pZ}{$8.77\mathrm{E}{-}15$}
\renewcommand{\pAA}{$7.70\mathrm{E}{-}15$}
\renewcommand{\pAB}{$7.70\mathrm{E}{-}15$}
\renewcommand{\pAC}{$0$}
\renewcommand{\pAD}{$0.00e+00$}
\renewcommand{\pAE}{$8.77\mathrm{E}{-}15$}
\renewcommand{\pAF}{$8.77\mathrm{E}{-}15$}
\renewcommand{\pAG}{$7.70\mathrm{E}{-}15$}
\renewcommand{\pAH}{$7.70\mathrm{E}{-}15$}
\renewcommand{\pAI}{$0.00e+00$}
\renewcommand{\pAJ}{$0$}


% Energies second gradient material, order 2, [4 8 16] Elements
% sorting: 4-diri & 4-peri & 8-diri & 8-peri & 16-diri & 16-peri
% \pA = abs(E(4-diri)-E(4-diri)) / E(4-diri)
% \pB = abs(E(4-diri)-E(4-peri)) / E(4-diri)

\renewcommand{\pA}{$0$}
\renewcommand{\pB}{$1.52\mathrm{E}{-}06$}
\renewcommand{\pC}{$8.43\mathrm{E}{-}09$}
\renewcommand{\pD}{$1.53\mathrm{E}{-}06$}
\renewcommand{\pE}{$2.60\mathrm{E}{-}08$}
\renewcommand{\pF}{$1.53\mathrm{E}{-}06$}
\renewcommand{\pG}{$1.52\mathrm{E}{-}06$}
\renewcommand{\pH}{$0$}
\renewcommand{\pI}{$1.51\mathrm{E}{-}06$}
\renewcommand{\pJ}{$6.94\mathrm{E}{-}09$}
\renewcommand{\pK}{$1.49\mathrm{E}{-}06$}
\renewcommand{\pL}{$1.43\mathrm{E}{-}08$}
\renewcommand{\pM}{$8.43\mathrm{E}{-}09$}
\renewcommand{\pN}{$1.51\mathrm{E}{-}06$}
\renewcommand{\pO}{$0$}
\renewcommand{\pP}{$1.52\mathrm{E}{-}06$}
\renewcommand{\pQ}{$1.75\mathrm{E}{-}08$}
\renewcommand{\pR}{$1.53\mathrm{E}{-}06$}
\renewcommand{\pS}{$1.53\mathrm{E}{-}06$}
\renewcommand{\pT}{$6.94\mathrm{E}{-}09$}
\renewcommand{\pU}{$1.52\mathrm{E}{-}06$}
\renewcommand{\pV}{$0$}
\renewcommand{\pW}{$1.50\mathrm{E}{-}06$}
\renewcommand{\pX}{$7.36\mathrm{E}{-}09$}
\renewcommand{\pY}{$2.60\mathrm{E}{-}08$}
\renewcommand{\pZ}{$1.49\mathrm{E}{-}06$}
\renewcommand{\pAA}{$1.75\mathrm{E}{-}08$}
\renewcommand{\pAB}{$1.50\mathrm{E}{-}06$}
\renewcommand{\pAC}{$0$}
\renewcommand{\pAD}{$1.51\mathrm{E}{-}06$}
\renewcommand{\pAE}{$1.53\mathrm{E}{-}06$}
\renewcommand{\pAF}{$1.43\mathrm{E}{-}08$}
\renewcommand{\pAG}{$1.53\mathrm{E}{-}06$}
\renewcommand{\pAH}{$7.36\mathrm{E}{-}09$}
\renewcommand{\pAI}{$1.51\mathrm{E}{-}06$}
\renewcommand{\pAJ}{$0$}
